Geometric Priors for Scientific Generative Models in Inertial Confinement Fusion

In this paper, we develop a Wasserstein autoencoder (WAE) with a hyperspherical prior for multimodal data in the application of inertial confinement fusion. Unlike a typical hyperspherical generative model that requires computationally inefficient sampling from distributions like the von Mis Fisher, we sample from a normal distribution followed by a projection layer before the generator. Finally, to determine the validity of the generated samples, we exploit a known relationship between the modalities in the dataset as a scientific constraint, and study different properties of the proposed model.

==> sections/background.tex <==
%%% THIS IS PLACEHOLDER TEXT FROM OUR NEURIPS 2019 WORKSHOP PAPER
Inertial confinement fusion (ICF) \cite{lindl1995development} experiments  use powerful lasers to heat and compress a millimeter-scale target filled with thermonuclear deuterium-tritium (DT) fuel.  The goal is to drive fusion reactions that self-heat the DT fuel leading to ignition and propagating burn.  The experiments employ a variety of diagnostic instruments to observe the fusion implosions.  These include exceptionally fast x-ray cameras and neutron cameras that create spectrally resolved (i.e. hypercolor) images, as well as a host of spectrometers and radiochemical diagnostics that produce key scalar features.  The fusion science teams use this multimodal set of observations as feedback to optimize the driving conditions of the experiment in a quest to improve the implosion performance.
 
Traditionally, ICF scientists use predictive forward models to produce simulated diagnostic output, which they later compare with experiments.  Recent work has used inference methods using deep neural networks as surrogates for the complicated radiation hydrodynamics codes that map laser and target conditions into output physics observations of images and scalars.  However, our physics application demands that the deep neural networks provide outputs that are consistent with physical laws, that constrain these outputs by establishing necessary functional relationships amongst them.  We formulate these scientific priors for all of the data modalities, providing us with individual priors amongst the scalars, priors amongst the images, and finally priors on relationships between images and scalars. As an example in this work, we can use notions of thermal equilibrium to relate predicted ion temperatures (as part of the scalars) to estimates of electron temperature formed by ratios of x-ray image brightnesses. As shown in the experiments, this manifests as a strong linear relationship between the predicted scalar, and the mean brightness of the x-ray images.  This constraint, and others allow us to judge the physical plausibility of DNN model predictions.  Those predictions that satisfy our ion/electron temperature requirements are admissible; those that violate them are ruled unphysical.

==> sections/conclusion.tex <==

In this work we utilized hypersphercial paramerization of the latent space in generative models for scientific data.

==> sections/proposedwork.tex <==
As mentioned earlier, we explore the use of a hyper-spherical embedding inside the generator while keeping the latent space Euclidean. This allows us to place a prior over the latent space using a standard Normal distribution which is easy to sample from, as opposed to more complex distributions such as the von Mises-Fisher (vMF). In doing so, we exploit the fact that a normal distribution projected onto to a hypersphere forms a uniform distribution on its shell. We demonstrate a proof of concept by extending the Wasserstein Autoencoder (WAE)\cite{tolstikhin2018wasserstein} with an additional layer that projects the latent vector obtained from the encoder onto a unit hypersphere. 

We define a unit hypersphere as $\mathcal{S}^{d-1} = \{\textbf{x} \in \mathbb{R}^d: ||\mathbf{x}||_2=1\}$. Our proposed model consists of the following: an encoder network, $\mathcal{E}: (\mathbf{I},\mathbf{S}) \rightarrow \mathbf{z}$; where $\mathbf{I}$ denotes a the multi-channel spectral image and $\mathbf{S}$ denotes the set of scalar diagnostics such as temperature, energy yield, pressure etc. To account for the multi-modal nature of the data, we use convolutional layers to process the image channels, and a fully connected layer to process the scalars. These are then stacked after a few layers before jointly predicting the bottleneck representation, $\mathbf{z}$.  Next, we define a projection map $\mathcal{P}: \mathbf{z} \rightarrow \mathcal{S}^{d-1}$, followed by a generator network $\mathcal{G}: S^{d-1} \rightarrow \mathbf{I}, \mathbf{S}$. Here the projection map $\mathcal{P}$ is defined as $\mathcal{P}(\mathbf{z})= \mathbf{z}/||\mathbf{z}||_2$. Thus, the encoder-decoder pair mapping is given by: $(\mathbf{I},\mathbf{S}) \xrightarrow[]{\mathcal{E}} \mathbf{z} \xrightarrow[]{\mathcal{P}} \mathbf{\tilde{z}} \xrightarrow[]{\mathcal{G}} (\mathbf{I},\mathbf{S})$.

We keep the discriminator from the standard Euclidean WAE unchanged, and use an adversarial cost to get the latent space $\mathbf{z}$ to match the prior distribution, which in our case is the zero mean unit variance Normal distribution, $\mathcal{N}(\mathbf{0},\mathbf{\mathrm{I}})$. During training, there are two key procedures that need to be taken into account--the generator is only fed samples from the hypersphere and the discriminator samples from the Euclidean Gaussian prior. This makes our approach simple to optimize as opposed to models with explicit hyperspherical distribution.

%The proposed approach builds on standard WAE and employs hyperspherical parametrization. We propose to transform the latent space to spherical manifold, before feeding it to the generator, thus forcing the latent space to the surface of unit hypersphere. 
%As opposed to existing methods that instead use von Mises-Fisher distribution to achieve hyperspherical latent spaces, that is not only inefficient due to rejection sampling procedure but also poses challenges in backpropagation, our sampling strategy is simple.
%This makes our approach purely geometric and free from any sophisticated sampling strategy. 





% Here we have no any probabilistic constraint on z

% \emph{i.e.}:

% \begin{equation}
%   \text{ For samples coming from encoder:}  \mathbf{z} \xrightarrow[]{Disc} y
%   \text{}
% \end{equation}

% The normal distribution of mean $\mu$ and covariance $\Sigma$ gets transformed to a uniform distribution on the hypersphere. 



